Emora: An Inquisitive Social Chatbot Who Cares For You

Inspired by studies on the overwhelming presence of experience-sharing in human-human conversations, Emora, the social chatbot developed by Emory University, aims to bring such experience-focused interaction to the current field of conversational AI. The traditional approach of information-sharing topic handlers is balanced with a focus on opinion-oriented exchanges that Emora delivers, and new conversational abilities are developed that support dialogues that consist of a collaborative understanding and learning process of the partner's life experiences. We present a curated dialogue system that leverages highly expressive natural language templates, powerful intent classification, and ontology resources to provide an engaging and interesting conversational experience to every user.

==> nlp/TopicIntent.tex <==

\begin{figure*}[htbp]
\includegraphics[width=400pt]{figures/TopicIntentEmora.png}
\caption{Flowchart of Emora topic and intent classifier. The blue rectangles are the final decisions, where Global and Local topic switch dialogue acts represent topic switch within a component and between components.}
\label{fig:TopicIntent}
\end{figure*}


To infer a user's intent in an Natural Language Understanding (NLU) component, the first stages entail the topic and dialogue act classification. In open-domain conversational agents, topic and dialogue act classification can be treated as a text classification problem \citep{rf:emerson, ahmadvand2018emory}. However, compared to general text classification, utterance classification poses a greater challenge due to four main factors: 1) the tendency of human utterances to be short; 2) errors in Automatic Speech Recognition (ASR); 3) users’ frequently mentioned out-of-vocabulary words and entities; and 4) lack of available labeled open-domain human-machine conversation data \citep{rf:CDAC, rf:concet}. 


Moreover, natural conversations entail utterances which are dependent on the context, thus making it impossible to classify the topic and intent without considering the preceding utterances. For example, when a user uses the expression, ``Oh, yeah'' it can be interpreted as one of the multiple options: "Reject-Disagree," "Accept-Agree," or "Topic-Switch." To help address these problems, in Emora, we developed a contextual-aware topic and dialogue act classification model for open-domain conversational agents.

To identify both {\em topic} and {\em dialogue acts}, we followed the latest research, as well as {\em Cobot} topic and dialogue act classifiers from Amazon. To achieve the task of identification, we developed a mixture of experts model that uses Cobot classifiers as experts to make the final decision. To this end, we developed our own topic and dialogue act classifier, which were trained on the internal datasets. Also, the customized classifiers are the deep learning models that we developed for last year's completion, and the details regarding implementation are described in \citep{ahmadvand2018emory}. The customized classifiers cover customized topics that Cobot does not cover and also tries to improve the quality of some specific classes. For example, we train our classifiers on new topics and dialogue acts such as ``Food-Drinks'', ``Travel-Geo'', and ``Yes-Answers.''  Also, to improve the accuracy of some classes like ``topic-switch'', we collected an internal dataset and trained our dialogue act classifier on this specific class to enhance the Cobot prediction. Figure \ref{fig:TopicIntent} shows a general flow of the Emora's topic and dialogue act classifiers, where Cobot classifier plays a principal role in the classification.  One of the significant shortcomings of the Cobot dialogue act classifier is that it provides one label for topic switching within and between topics. We notice that Cobot dialogue act classifier offers a high precision on the global topic switching between two topics (e.g., {\em Music} to {\em Movie}). However, this topic switching is often local and happens inside a specific topic like {\em Music}. For instance, when a user says, ``no, I don't like Taylor Swift songs, let's talk about Drake''; this is a local topic switch. However, ``I am bored of music, how about current Disney animations'' represents a global topic switch where the user wants to talk about another topic. We also define a new state named ``Followup'' where the user is interested in the current topic and want to keep talking about that specific topic. For both local ``topic\_switch'' and ``Followup'' user intends to stick with the ongoing conversation topic, two different conversation strategies need to be planned to continue the conversation.





==> nlp/evi.tex <==
\paragraph{EVI}



==> nlp/namedentity.tex <==
Named entities are identified within user utterances using the spaCy Named Entity Recognition (NER) service\footnote{https://spacy.io/usage/linguistic-features\#named-entities}. SpaCy NER is a statistical model trained on the OntoNotes 5 corpus which recognizes 18 classes of named entities, including \textit{person}, \textit{organization}, and \textit{location}.

==> nlp/sentiment.tex <==
We use the Valence Aware Dictionary and sEntiment Reasoner (VADER) to provide a sentiment score for each received user utterance (\cite{hutto:14}). VADER is specifically tuned for social media and microblog content, which is applicable to the casual, short nature of dialogue utterances, and provides low latency due to the rule-based lexicon formulation of the VADER model.
